Conformance Testing for Stochastic Cyber-Physical Systems

Conformance is defined as a measure of distance between the behaviors of two dynamical systems. The notion of conformance can accelerate system design when models of varying fidelities are available on which analysis and control design can be done more efficiently. Ultimately, conformance can capture distance between design models and their real implementations and thus aid in robust system design. In this paper, we are interested in the conformance of stochastic dynamical systems. We argue that probabilistic reasoning over the distribution of distances between model trajectories is a good measure for stochastic conformance. Additionally, we propose the non-conformance risk to reason about the risk of stochastic systems not being conformant. We show that both notions have the desirable transference property, meaning that conformant systems satisfy similar system specifications, i.e., if the first model satisfies a desirable specification, the second model will satisfy (nearly) the same specification. Lastly, we propose how stochastic conformance and the non-conformance risk can be estimated from data using statistical tools such as conformal prediction. We present empirical evaluations of our method on an F-16 aircraft, an autonomous vehicle, a spacecraft, and Dubin's vehicle.

==> ArXiv_version/chapter/attic.tex <==
\subsection{Introduction to Conformal Inference}

Conformal inference, as proposed in works such \cite{vovk2005algorithmic,shafer2008tutorial}, is a framework that allows for the generation of high-confidence prediction regions for any prediction algorithm. It does not make assumptions about the distribution of the input data to the framework and is able to maintain a high confidence level for the prediction regions, regardless of the amount of data provided.

Our goal is to construct a prediction region for $d(x,x')$ that is defined by a fixed value of $C$ such that
% \begin{equation}\label{eq:goal01}
%     \forall x \in \mathcal{D}  \forall x' \in \mathcal{D'}, 
%     P \big( d(x, x') \leq C \big) \geq 1 - \delta 
% \end{equation}
% can change to the i notation.

\begin{equation}\label{eq:goal01}
    P \big( \sup_{u \in U} d(x, x') \leq C \big) \geq 1 - \delta 
\end{equation}
We approximate the goal by
\begin{equation}\label{eq:goal01}
    P \big( \sup_{u \sim D_U} d(x, x') \leq C \big) \geq 1 - \delta 
\end{equation}
% reverse compute x'?

To find the value of constant $C$, we evaluate the nonconformity score of $R$, which is defined as $R:=d(x, x')$. We compute the nonconformity score for each validation trajectory $(x^{(i)}, x'^{(i)}) \in D_{val} \times D'_{val}$ as  
\begin{equation}
    R^{(i)} := d(x^{(i)}, x'^{(i)})
\end{equation}

Conformal inference guarantees that with probability $1 - \delta$, the distance between the trajectories of two systems will be no greater than $C$.

\subsection{Conformance checking for stochastic systems}


%old 
% \begin{problem}\label{prob01}
% Given a distance metric $d$, two trajectory distirubtions  $(X_0,X_1,\hdots)\sim\mathcal{D}$,  $(X'_0,X'_1,\hdots)\sim\mathcal{D'}$, the observations $x_{\text{obs}}:=(x_0,\hdots,x_t)$, a target distance $\epsilon$ and a failure probability $\delta \in (0,1)$, determine if $\forall x^{(i)} \in \mathcal{D}  \forall x'^{(i)} \in \mathcal{D'}, P\big(d(x^{(i)}, x'^{(i)}) \leq \epsilon \big) \geq 1 - \delta$ holds.
% \end{problem}



Note that we do not place any restrictions on the control signal or input parameters; all possible behaviors of the two systems are taken into account. In this case, $\epsilon$ represents the maximum possible distance between the two systems, with confidence $1 - \delta$. Now let us consider if $x^{(i)}$ and $x'^{(i)}$ capture the output of the system for all possible input signals and stochastic inside the system. 

\begin{problem}\label{prob01}
Given a distance metric $d$, two trajectory distirubtions  $(X_0,X_1,\hdots)\sim\mathcal{D}$,  $(X'_0,X'_1,\hdots)\sim\mathcal{D'}$, the observations $x_{\text{obs}}:=(x_0,\hdots,x_t)$, a target distance $\epsilon$ and a failure probability $\delta \in (0,1)$, determine if $ P\big(\sup_{u \sim D_U} d(x^{(i)}, x'^{(i)}) \leq \epsilon \big) \geq 1 - \delta$ holds.
\end{problem}










\subsubsection{Brute-force conformance}
We can achieve coverage by using brute-force sampling. We randomly select a set of $M$ potential inputs $U$, and for each input $u \in U$, we run simulations of each system $N$ times. This results in $M \times N$ output trajectories. By using conformal inference on the resulting output trajectories, we can determine the maximum distance between the two systems.

\begin{theorem}\label{thm:force}
Given a distance metric $d$, two trajectory distirubtions  $(X_0,X_1,\hdots)\sim\mathcal{D}$,  $(X'_0,X'_1,\hdots)\sim\mathcal{D'}$, the observations $x_{\text{obs}}:=(x_0,\hdots,x_t)$, a target distance $\epsilon$, two datasets $D_\text{val}$, $D'_\text{val}$, and a failure probability $\delta \in (0,1)$, Then the prediction regions in equation  \eqref{eq:goal01} are valid with $C_i$ defined as
\begin{align}\label{eq:thm_1}
    C:=R^{(p)}\;\;\text{where}\;\;  p:=\big\lceil (|D_\text{val}|\cdot|D'_\text{val}|+1)(1-\delta)\big\rceil,
\end{align}
\end{theorem}

\subsubsection{Robust conformance}
Another way to approach this is by using conformal prediction in two stages. In the first stage, we predict the maximum distance $\epsilon_d^u$ between the two systems for each sampled input signal. In the second stage, rather than using $N$ simulations for each input signal $u$, $N$ signals are specifically constructed within distance $\epsilon_d^u$ of the signal $u$. In this case, we can ensure the performance even when the samples do not fully reflect the actual distribution of the output trajectory.


We compute the expected nonconformity score for each validation trajectory $(x^{(i)}_n, x'^{(i)}_n) \in D_{val}^i \times D'^i_{val}$ with $N$ being the simulation time as  %todo: notation here 
\begin{equation}
\begin{split}
    R_n^{(i)} & := d(x^{(i)}_n, x'^{(i)}_n) \\
    E(R_n^{(i)}) & := \frac{1}{N}\sum_{n = 1}^N d(x^{(i)}_n, x'^{(i)}_n)  \text{(not used)}
\end{split}
\end{equation}

Conformal inference guarantees that with probability $1 - \delta$, the distance between the trajectories of two systems given an input signal $u$, will be no greater than $C$.

\begin{lemma}[\cite{stankeviciute2021conformal,lindemann2022safe}]\label{lem:01}Given a distance metric $d$, two trajectory distirubtions  $(X_0,X_1,\hdots)\sim\mathcal{D}$,  $(X'_0,X'_1,\hdots)\sim\mathcal{D'}$, the observations $x_{\text{obs}}:=(x_0,\hdots,x_t)$, a target distance $\epsilon$, two datasets $D_\text{val}$, $D'_\text{val}$, and a failure probability $\delta \in (0,1)$, Then the prediction regions in equation  \eqref{eq:goal01} are valid with $C_i$ defined as
\begin{align}\label{eq:lem_1}
    C_i:=R_i^{(p)}\;\;\text{where}\;\;  p:=\big\lceil (|D_\text{val}^i|\cdot |D'^i_\text{val}|+1)(1-\bar{\delta})\big\rceil \text{ and } \bar{\delta}:=\delta/N.
\end{align}
\end{lemma}

If for each input signal, the distance is bounded, then for all possible input signal, the distance shall also be bounded. We use $C_i$ to construct a tube for $x^{(i)'}$ and substitute $\mathcal{D'}$ in equation \eqref{eq:goal01} with $D'_{C_i}$  %?  
Then we can reason about
\begin{equation}\label{eq:goal01}
    \forall x \in \mathcal{D}  \forall x' \in \mathcal{D'}_{C_i}, 
    P \big( d(x, x') \leq C \big) \geq 1 - \delta 
\end{equation}

Then robust conformal? $d(x, x')$ to $d(x, x'_{C_i})$? and $C$ to $C'$?

% each initial state has distance d,
% worst case M * d, is the largest distance. 
% where M is the number of possible input signal (control signal)



% use conformal to get worst input signal?


\section{Transference between system}
Given the two systems are $(\delta, \epsilon)$-close, we apply the verification results from one system to the other. We compare the verification results on a region-by-region basis.

% \begin{lemma}[Theorem 1 in~\cite{donzeRobustSatisfactionTemporal2010}]
% \label{lem:robust_satisfaction_nearby_secondaries} 
% If \(\rho^\varphi(x, t) = \delta\), then for every signal \(x'\) satisfies \(||x - x'|| < \delta\), then 
% \((x \models \varphi) \implies (x' \models \varphi)\).
% \end{lemma} (goes into related work)

\begin{theorem} [Transference for Traces] 
Let $x^{(i)}, x'^{(i)}$ be realizations of distribution $\mathcal{D}$ and $\mathcal{D'}$, and $d (x^{(i)}, x'^{(i)}) \leq \epsilon$. Let $\phi$ be a bounded STL formula, we have $x^{(i)} \models \phi \implies x'^{(i)} \models \phi$
\end{theorem}



\section{Conformal Prediction for Predictive Runtime Verification}

In this section, we first provide an introduction to conformal prediction for uncertainty quantification. We then propose two predictive runtime verification algorithms to solve Problem \ref{prob1}. We refer to these algorithms as direct and indirect. This naming convention is motivated as the direct method applies conformal prediction directly to obtain a prediction region for the robust semantics $\rho^{\phi}(X,\tau_0)$. The indirect method uses conformal prediction to get prediction regions for future states $X_\tau$ first, which are subsequently used indirectly to obtain a prediction region for $\rho^{\phi}(X,\tau_0)$, see Figure \ref{fig:11}.





\subsection{Introduction to Conformal Prediction}
\label{sec:intro_conf}
Conformal prediction was introduced  in \cite{vovk2005algorithmic,shafer2008tutorial} to obtain valid prediction regions for complex prediction algorithms, i.e., neural networks, without making assumptions on the underlying distribution or the prediction algorithm \cite{angelopoulos2021gentle,zeni2020conformal,lei2018distribution,tibshirani2019conformal,cauchois2020robust}.  We first provide a brief introduction to conformal prediction. 

Let $R^{(0)},\hdots,R^{(k)}$ be $k+1$ independent and identically distributed random variables. The variable $R^{(i)}$ is usually referred to as the {nonconformity score}. In supervised learning, it may be defined as $R^{(i)}:=\|Y^{(i)}-\mu(X^{(i)})\|$ where the predictor $\mu$ attempts to predict an output  $Y^{(i)}$ based on an input $X^{(i)}$.  A large nonconformity score indicates a poor predictive model. 

Our goal is to obtain a prediction region for $R^{(0)}$ based on $R^{(1)},\hdots,R^{(k)}$, i.e., the random variable $R^{(0)}$ should be contained within the prediction region with high probability.  Formally, given a failure probability $\delta\in (0,1)$, we want to construct a valid prediction region $C$ that depends on $R^{(1)},\hdots,R^{(k)}$ such that 
\begin{align*}
    P(R^{(0)}\le C)\ge 1-\delta.
\end{align*}

As $C$ depends on $R^{(1)},\hdots,R^{(k)}$, note that the probability measure $P$ is defined over the product measure of $R^{(0)},\hdots,R^{(k)}$.
By a surprisingly simple quantile argument, see \cite[Lemma 1]{tibshirani2019conformal}, one can obtain $C$ to be the $(1-\delta)$th quantile of the empirical distribution of the values $R^{(1)},\hdots,R^{(k)}$ and $\infty$. By assuming that $R^{(1)},\hdots,R^{(k)}$ are sorted in non-decreasing order, and by adding $R^{(k+1)}:=\infty$, we can equivalently obtain $C:=R^{(p)}$ where $p:=\lceil (k+1)(1-\delta)\rceil$, i.e., $C$ is the $p$th smallest nonconformity score.




==> ArXiv_version/chapter/attic_tables.tex <==
\section{Dubin Case study performance}

\begin{equation}
\begin{split}
        \phi_1 &= G(|c_e| \leq 2.25) \\
        \phi_2 &=  G_{[10, \infty)} (|c_e| \leq 2.25)\\
        \phi_3 &= F_{[0,5]}G_{[0,5]} ( |c_e| \leq 1.25)  \\
        \phi_4 &= G_{[10, \infty)}(|c_e| \geq 1.25) \implies F_{[0, 5]}G_{[0, 5]} |c_e| \leq 1.25)
\end{split}
\end{equation}


\begin{figure}[]
\centering
\subfloat[Distance on training set]{
\includegraphics[scale=0.23]{ArXiv_version/figures_case_studies/dubin/R_hist_dsig_scorenum1000_sup_norm_delta0.05_Trainratio0.200.png}\label{subfig:dist_train}}
\hfill
\subfloat[Robustness on train set controller one]{
\includegraphics[scale=0.23]{ArXiv_version/figures_case_studies/dubin/R_hist_rho_ctl1_scorenum1000_sup_norm.png}\label{subfig:rho_ctl1_train}}
\hfill
\subfloat[Robustness on train set controller two]{
\includegraphics[scale=0.23]{ArXiv_version/figures_case_studies/dubin/R_hist_rho_ctl2_scorenum1000_sup_norm.png}\label{subfig:rho_ctl2_train}}
\hfill
\subfloat[Distance on test set]{
\includegraphics[scale=0.23]{ArXiv_version/figures_case_studies/dubin/test_R_hist_dsig_scorenum1000_sup_norm_delta0.05_trainnum1000.000.png}\label{subfig:dist_test}}
\hfill
\subfloat[Robustness on test set controller one]{
\includegraphics[scale=0.23]{ArXiv_version/figures_case_studies/dubin/test_R_hist_rho_ctl1_scorenum1000_sup_norm.png}\label{subfig:rho_ct1_test}}
\hfill
\subfloat[Robustness on test set controller two]{
\includegraphics[scale=0.23]{ArXiv_version/figures_case_studies/dubin/test_R_hist_rho_ctl2_scorenum1000_sup_norm.png}\label{subfig:rho_ct2_test}}

\caption{Distance and Robustness histogram for Dubin Case study. $\delta_1=\delta_2=0.05$. Fig \ref{subfig:dist_train} shows the distance distribution of training data between the two systems. Fig \ref{subfig:dist_test} shows the distribution of distance on the test data. Fig \ref{subfig:rho_ctl1_train} shows the robustness distribution of system one on training data. Fig \ref{subfig:rho_ct1_test} shows the distribution of rho on test data for system one. Fig \ref{subfig:rho_ctl2_train} shows the robustness distribution on training data for system 2. Fig \ref{subfig:rho_ct2_test} shows the robustness distribution on test data for system 2. }\label{fig:dubin_hist}
\end{figure}



\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline &
  \begin{tabular}[c]{@{}l@{}} Calibration size \\ $/$ Test size \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Time  \\ $\rho_1$  (s)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Time \\ $\epsilon$  (s)\end{tabular} &
  V.S. $\rho_1$ &
  V.S. $d(y1,y2)$ &
  V.S. transfer \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\delta_1$ =0.2\\ $\delta_2$= 0.05\end{tabular}}  & $100 / 1000$ & 0.0 &0.0 &0.956 &0.767 &1.0 \\ \cline{2-7}    & $3000 / 1000$ &0.001&0.0&0.952&0.792&1.0  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\delta_1$=0.1\\ $\delta_2$= 0.05\end{tabular}} & $1000 / 1000$ & 0.0&0.0&0.957&0.918&1.0  \\ \cline{2-7} & $3000 / 1000$ & 0.001& 0.0& 0.952& 0.906& 1.0  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\delta_1$=0.05\\ $\delta_2$=0.05\end{tabular}}   & $2000 / 1000$ &0.001& 0.0& 0.942& 0.952& 1.0 \\ \cline{2-7} 
& $3000 / 1000$ & 0.001& 0.0& 0.952& 0.952& 1.0  \\ \hline
\end{tabular}
\caption{Time consumption and V.S. with different set up of $\delta$ on case study dubin}
\end{table}


\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Case Studies &
  \begin{tabular}[c]{@{}l@{}} Calibration size \\ $/$ Test size \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Time  \\ $\rho_1$  (s)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Time\\ $\epsilon$ (s)\end{tabular} &
  V.S. $\rho_1$ &
  V.S. $d(y1,y2)$ &
  V.S. transfer \\ \hline
$\phi_1$   & $700/300$ & 0.015 &0.0 &0.94 &0.9567 &1.0   \\ \hline
$\phi_2$ & $700/300$ &0.013& 0.0& 0.94& 0.9567& 1.0  \\ \hline
$\phi_3$      & $700/300$ & 1.5323& 0.0& 0.9467& 0.9567& 1.0  \\ \hline
$\phi_4$   &  $700/300$ & 7.2076&0.0&0.95&0.9567 & N/A    \\ \hline
% $\phi_5$     & $700/300$ &15.9105&0.0&0.9267&0.9567& 1.0    \\ \hline
\end{tabular}
\caption{CARLA with different specifications $\delta_1=0.05$, $\delta_2=0.05$}
\end{table}


\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Distance \\ methods\end{tabular} &
  \begin{tabular}[c]{@{}l@{}} Calibration size \\ $/$ Test size \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} Conformal \\ Value $\epsilon_d$ \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Validation Score \\ (V.S.)  for d(y1, y2) \end{tabular} &
    \begin{tabular}[c]{@{}l@{}} VaR for \\ d(y1, y2) \end{tabular} &
        \begin{tabular}[c]{@{}l@{}}CVaR for \\ d(y1, y2) \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Time for \\ Calculating \\distance (s)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Time for\\  conformal (s)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Total \\time  (s)\end{tabular} \\ \hline
\multirow{5}{*}{Sup norm}  & $50/1000$ &0.7825&0.987&0.7183 &0.7947&0.0&0.0&0.0 \\ \cline{2-9} 
            & $100/1000$  &0.7313& 0.959&0.7282 &0.7626& 0.0& 0.001& 0.001 \\ \cline{2-9} 
            & $500/1000$  & 0.6982 &0.93 &0.695&0.7433 &0.002 &0.0 &0.002 \\  \cline{2-9} 
   & $1000/1000$  & 0.7163 &0.956&0.7148&0.7647 &0.005 &0.0 &0.005 \\ \cline{2-9} 
  & $2000/1000$& 0.7122 &0.952 &0.712&0.7814 &0.009 &0.0 &0.009 \\ \cline{2-9}
   & $3000/1000$ & 0.7118 & 0.952 &0.7117 &0.7862&0.014 & 0.001 & 0.015
   \\
   \hline
\multirow{5}{*}{Skorokhod} & $50/1000$   &  &&    &  &        &       &        \\ \cline{2-9} 
                           & $100/1000$  &    &&   & &        &       &        \\ \cline{2-9} 
                           & $500/1000$  &     &&  & &        &       &        \\  \cline{2-9} 
 & $1000/1000$  &       & &        &       &     &&   \\  \cline{2-9}
 & $2000/1000$  &       & &        &       &       && \\  \cline{2-9}
  & $3000$/$1000$  &       & &        &       &      &&  \\
 \hline
\multirow{5}{*}{L2 norm}  & $50/1000$ &2.6086&0.937&2.503&2.6119&0.001 &0.0&0.001 \\ \cline{2-9} 
            & $100/1000$  &2.5901&0.936&2.5497 & 2.7397&0.001&0.0&0.001 \\ \cline{2-9} 
            & $500/1000$  & 2.5475&0.934&2.5278&2.904&0.003&0.0&0.003 \\  \cline{2-9} 
   & $1000/1000$  & 2.7339&0.96&2.7317&2.7317&0.005&0.0&0.005 \\ \cline{2-9} 
     & $2000/1000$& 2.7071 &0.944&2.7059&3.0436 &0.009 &0.0 &0.009 \\ \cline{2-9}
   & $3000/1000$ & 2.7238&0.955&2.722&3.0929&0.015&0.0&0.015
   \\
   \hline
\end{tabular}
\caption{Complexity of doing conformance, $\delta_1=\delta_2=0.05$. On case study Dubin}
\end{table}



\begin{figure}[t]
\centering
\subfloat[CARLA case study trajectories]{
\includegraphics[width=0.35\linewidth]{ArXiv_version/figures_case_studies/trajs/carla_traj.png}\label{carla_traj}}
\subfloat[Dubin]{
\includegraphics[width=0.35\linewidth]{ArXiv_version/figures_case_studies/trajs/dubin.png}\label{dubin_traj}}
\hfill
\subfloat[Quad Rotor]{
\includegraphics[width=0.35\linewidth]{ArXiv_version/figures_case_studies/trajs/quadrotor.png}\label{quad_traj}}
\subfloat[Satelite data]{
\includegraphics[width=0.35\linewidth]{ArXiv_version/figures_case_studies/trajs/satelite.png}\label{sat_traj}}
\subfloat[F16 data]{
\includegraphics[width=0.35\linewidth]{ArXiv_version/figures_case_studies/trajs/f16.png}\label{f16_traj}}
\caption{Trajectories from two systems on different case studies}\label{fig:system_trajs}
\end{figure}




\begin{table}[]
\centering
\begin{tabular}{llllllll}
\hline &
  \begin{tabular}[c]{@{}l@{}} Calibration size \\ $/$ Test size \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} $Conf(-\rho(Y_1))$   \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} $Conf(d(Y_1,Y_2))$ \\ \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} V.S. \\$Conf(-\rho(Y_1))$  \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} V.S. \\ $Conf(d(Y_1,Y_2))$ 
   \end{tabular} &
   \begin{tabular}[c]{@{}l@{}} 
   V.S. \\
   transfer \end{tabular} &
    \begin{tabular}[c]{@{}l@{}} $Conf(-\rho(Y_2))$ \end{tabular}
  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\delta_1$ =0.2\\ $\delta_2$= 0.05\end{tabular}}  & $1000 / 3000$ & 0.1272  & 0.0142 & 0.968 & 0.7977 & 0.983 & -0.5506 \\ \cline{2-8}    & $7000 / 3000$ & 0.0879 & 0.0141 &0.953&0.8113&0.988 & -0.5341  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\delta_1$=0.1\\ $\delta_2$= 0.05\end{tabular}} & $2000 / 3000$ & 0.0631 &0.0167 &0.949 &0.89 &0.993 &-0.4543 \\ \cline{2-8} & $7000 / 3000$ & 0.0879 & 0.0169 & 0.953 & 0.9083 & 0.989 & -0.4219  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\delta_1$=0.05\\ $\delta_2$=0.05\end{tabular}}   & $3000 $/$ 3000$ & 0.0442 & 0.0196& 0.944 & 0.95 & 0.9957 & -0.3674  \\ \cline{2-8} 
& $7000 / 3000$ & 0.0879& 0.0195 & 0.953& 0.9517& 0.9891 & -0.3420 \\ \hline
\end{tabular}
\caption{Conformal performance evaluation with different $\delta$ on case study QuadRotor}\label{tb:quad_exp1}
\end{table}



\begin{table}[]
\centering
\begin{tabular}{llllll}
\hline &
  \begin{tabular}[c]{@{}l@{}} Calibration size \\ $/$ Test size \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} CVaR for \\ $d(Y_1, Y_2)$  \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} CVaR for \\ $- \rho(Y_1)$  \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} CVaR for \\ $- \rho(Y_2)$ \end{tabular} &  V.S. transfer  2   \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\delta_1$ =0.2\\ $\delta_2$= 0.05\end{tabular}}  
& $1000 / 3000$ & 0.0283   & 0.365 & -0.1337 & Success \\ \cline{2-6}   
& $7000 / 3000$ &0.0296 &0.3194 & -0.1311& Success  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\delta_1$=0.1\\ $\delta_2$= 0.05\end{tabular}} & $2000 / 3000$ & 0.0235 &0.3047 & -0.1495 &Success  \\ \cline{2-6} & $7000 / 3000$ & 0.0242 & 0.3194 & -0.1311  & Success  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}$\delta_1$=0.05\\ $\delta_2$=0.05\end{tabular}}   & $3000 $/$ 3000$ & 0.0228 & 0.2934 & -0.1502 & Success  \\ \cline{2-6} 
& $7000 / 3000$ & 0.023& 0.3194&  -0.1311 & Success\\ \hline
\end{tabular}
\caption{ Transference non conformance risk on case study QuadRotor}\label{tb:nonconfm_risk_quad}
\end{table}


\begin{table}[]
\centering
\begin{tabular}{llllll}
\hline
\begin{tabular}[c]{@{}l@{}}Distance \\ methods\end{tabular} &
  \begin{tabular}[c]{@{}l@{}} Calibration size \\ $/$ Test size \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} Conformal \\ Value $Conf(d(Y_1, Y_2))$ \\$\epsilon_d$ \end{tabular} &
    \begin{tabular}[c]{@{}l@{}}Validation Score \\ (V.S.)  for $d(Y_1, Y_2)$ \end{tabular} &
    \begin{tabular}[c]{@{}l@{}} VaR for \\ $d(Y_1, Y_2)$ \end{tabular} &
        \begin{tabular}[c]{@{}l@{}}CVaR for \\ $d(Y_1, Y_2)$ \end{tabular} \\ \hline
\multirow{5}{*}{Sup norm} 
 & $100/3000$ &0.0224&0.977&0.0203 & 0.0248  \\ \cline{2-6} 
     & $1000/3000$  &0.0192&0.9367&0.019 & 0.0225  \\ \cline{2-6} 
     & $3000/3000$  & 0.0196 & 0.95 & 0.0196 & 0.0228  \\  \cline{2-6} 
   & $5000/3000$  & 0.0195 & 0.951& 0.0195 &0.023   \\ \cline{2-6} 
   & $7000/3000$ & 0.0195& 0.9517& 0.0195 & 0.023 
   \\
   \hline
\multirow{5}{*}{Skorokhod} & $100/3000$   &      &  &        &    \textcolor{green}{remove cvar?}           \\ \cline{2-6} 
                           & $1000/3000$  &      & &        &              \\ \cline{2-6} 
                           & $3000/3000$  &       & &        &               \\  \cline{2-6} 
 & 5000$/$3000  &       & &        &              \\  \cline{2-6}
  & 7000$/$3000  &              &       &     &   \\
 \hline
\multirow{5}{*}{L2 norm}   & $100/3000$   & 0.0503 & 0.9403 & 0.0491 & 0.0613  \\ \cline{2-6} 
& $1000/3000$  & 0.0496 &0.931 & 0.0495 & 0.059     \\ \cline{2-6} 
    & $3000/3000$  &  0.0515&0.9507&0.0515 & 0.0609  \\  \cline{2-6} 
   & $5000/3000$  & 0.0514 &0.949 & 0.0514 & 0.0612   \\ 
                           \cline{2-6} 
   & $7000/3000$ & 0.0515 & 0.9517& 0.0515 & 0.0612 
   \\\hline
\end{tabular}
\caption{Conformance performance $\delta_1=\delta_2=0.05$. On case study QuadRotor}\label{tb:qd_com}
\end{table}

==> ArXiv_version/chapter/table_with_bounds.tex <==
\begin{table}[]
\centering
\begin{tabular}{lllllll}
\hline
Case Studies           &       \begin{tabular}[c]{@{}l@{}} $|D_{cal}|$  \\ $/$ Test size \end{tabular}     &
$\gamma$ , $\delta$  &
\begin{tabular}[c]{@{}l@{}} $CVaR(d(Y_1, Y_2))$  \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} $CVaR(- \rho(Y_1))$  \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} $CVaR(- \rho(Y_2))$
  \end{tabular}   

& Risk Check \\ \hline
\multirow{2}{*}{Satelite}   & \multirow{2}{*}{$7000/3000$} & 0.05   &0.2157 &-0.001& 0.0645& Success    \\   &                       & 0.01  & 0.2319 & -0.0008  & 0.0799  & Success    \\ \hline
\multirow{2}{*}{Quad rotor} & \multirow{2}{*}{$7000/3000$} & 0.05  & 0.0454& -0.012 & 0.4095 & Success    \\   &                       & 0.01   &  0.0478 & 0.0488 &  0.5961 & Success    \\ \hline
\multirow{2}{*}{Dubin}      & \multirow{2}{*}{$1000/3000$} & 0.05   & 0.9467 & -0.1382 & 0.1771 & Success    \\  &                       & 0.01  &0.9958  &-0.1165 & 0.2454& Success    \\ \hline
\multirow{2}{*}{Carla}      & \multirow{2}{*}{$700/300$} & 0.05  & 2.4481 & -0.227& 0.787 &  Success\\   &             & 0.01     & 2.5004 & -0.1383 & 1.056& Success \\ \hline
\multirow{2}{*}{F16}        & \multirow{2}{*}{$1000/3000$} &  0.05   & 237.0323 & 201.9314 & 201.9314 &  Success  \\   &     & 0.01   & 236.2832 & 196.5383 &196.5383 & Success   \\ \hline
\end{tabular}
\caption{check theorem \ref{tb:nonconfm_risk} on risk for all case studies}\label{tb:5}
\end{table}
